Revising Partially Ordered Beliefs

This paper deals with the revision of partially ordered beliefs. It proposes a semantic representation of epistemic states by partial pre-orders on interpretations and a syntactic representation by partially ordered belief bases. Two revision operations, the revision stemming from the history of observations and the possibilistic revision, defined when the epistemic state is represented by a total pre-order, are generalized, at a semantic level, to the case of a partial pre-order on interpretations, and at a syntactic level, to the case of a partially ordered belief base. The equivalence between the two representations is shown for the two revision operations.

==> fig/fig0.tex <==
\begin{figure}[h]
\caption{Epistemic states and partial pre-orders}\label{map}
\vspace{3cm}
  \centering
%  \psgrid(0,0)(-2,-2)(2,2)
    \rput(-2,2){\rnode{n1}{$\preceq_{\Sigma}$}}
    \rput(2,2){\rnode{n2}{$\preceq_{\Psi}$}}
    \rput(-2,1){\rnode{n3}{$\preceq_{\Sigma \circ^{sy} \mu}$}}
    \rput(2,1){\rnode{n4}{$\preceq_{\Psi \circ^{se}\mu}$}}
    \rput(-2,0){\rnode{n5}{$Bel^{sy}(\Psi \circ^{sy} \mu)$}}
    \rput(2,0){\rnode{n6}{$Bel^{se}(\Psi \circ^{se} \mu)$}}
 
   
    \ncLine[nodesep=10pt]{->}{n1}{n2}\Aput{a}
    \ncline[nodesep=3pt]{->}{n1}{n3}\Aput{b}
    \ncline[nodesep=10pt]{->}{n2}{n4}
    \ncline[nodesep=3pt]{->}{n3}{n5}
    \ncline[nodesep=10pt]{->}{n3}{n4}
    \ncline[nodesep=3pt]{->}{n4}{n6}
    \ncline[nodesep=3pt]{<->}{n5}{n6}
\end{figure}



==> fig/fig6.tex <==
\begin{figure}[h]
  \caption{Representation of $\preceq_{\Psi,w}$}\label{ex<psi}
\vspace{2cm}
  \centering
%  \psframebox{
                                %    \psorigin(0,0)
    \rput(0,0){\rnode{I5}{$\omega_0=\omega_2=\omega_8=\omega_9=\omega_{10}=\omega_{11}=\omega_{12}=\omega_{13}$}}
    \rput(-2,1){\rnode{I1}{$\omega_1=\omega_3=\omega_4=\omega_6$}}
    %\rput(-1,1.5){\rnode{I2}{$\omega_4=\omega_6$}}
    \rput(2,1.5){\rnode{I3}{$\omega_5=\omega_7$}}
    \rput(-2,2){\rnode{I4}{$\omega_{14}=\omega_{15}$}}
    \ncline[nodesep=3pt]{<-}{I5}{I1}
    \ncline[nodesep=3pt]{<-}{I5}{I2}
    \ncline[nodesep=3pt]{<-}{I5}{I3}
    \ncline[nodesep=3pt]{<-}{I1}{I4}
%}
 

\end{figure}



==> fig/fig7.tex <==
\begin{figure}[h]
\caption{Representation of $we(\Sigma\syntax^{se}\mu)$}\label{exstmap}
\vspace{3cm}
  \centering
%  \psframebox{
                                %    \psorigin(0,0)
    \rput(0,1.5){\rnode{I5}{$\omega_0=\omega_2=\omega_8=\omega_{10}=\omega_{12}$}}
    \rput(0,2.25){\rnode{I1}{$\omega_4=\omega_6$}}
    \rput(0,3){\rnode{I4}{$\omega_{14}$}}

    \rput(0,0){\rnode{I9}{$\omega_9=\omega_{11}=\omega_{13}$}}
    \rput(-2,0.5){\rnode{I6}{$\omega_1=\omega_3$}}
    \rput(2,1){\rnode{I7}{$\omega_5=\omega_7$}}
    \rput(-2,1.25){\rnode{I8}{$\omega_{15}$}}



    \ncline[nodesep=3pt]{<-}{I9}{I6}
    \ncline[nodesep=3pt]{<-}{I9}{I7}
    \ncline[nodesep=3pt]{<-}{I6}{I8}
%}


    \ncline[nodesep=3pt]{<-}{I1}{I4}
    \ncline[nodesep=3pt]{<-}{I5}{I1}
    \ncline[nodesep=3pt]{<-}{I8}{I5}
    \ncline[nodesep=3pt]{<-}{I7}{I5}
\end{figure}



==> fig/figtmp.tex <==
\begin{figure}[h]
\caption{Representation of epistemic state $\Psi\syntax^{se}\mu$}\label{exsemi}
\vspace{0.4cm}
{\tiny
$
\setlength{\arraycolsep}{1cm}
\def\tX{\tilde{\tilde{X}}}
\begin{array}{cc}
        (X-A,N-A)\rnode{a}{} & \rnode{b}{}(\tX,a)\\[1.5cm]
        (X,N)\rnode{c}{} & \rnode{d}{}(\tX,N)\\[1.5cm]
\end{array}
\psset{nodesep=5pt,arrows=->}
%\onlySlide*{2}{\nccurve[linecolor=white,angleA=270,angleB=180]{LIEN}{d}}%
\ncline[linecolor=white]{a}{b}\Aput{a}
\ncline[linecolor=white]{a}{c}\Bput{r}
\ncline[linecolor=white,linestyle=dashed]{c}{d}\Bput{b}
\ncline[linecolor=white]{b}{d}\Bput{s}
$
%\end{equation*}}
%\end{slide}
}
\end{figure}



==> fig/tst.tex <==
\begin{figure}[h]
  \caption{Representation of initial epistemic state $\Psi$}\label{fig.initial}
\vspace{2cm}
  \centering

  \rput(0,0){\rnode{R6}={(b\land c\to\lnot a)\lor d}}
  \rput(0,0.75){\rnode{R5}{b\to a\lor d}}

  \rput(0,1.5){\rnode{R4}{d}}
  \rput(1,2.5){\rnode{R3}{d\to a}}
  \rput(-1,2.25){\rnode{R2}{b\land c\to\lnot a}}
  \rput(-1,2.3){\rnode{R1}{b\to a}}


  \ncline[nodesep=3pt]{<-}{R6}{R5}
  \ncline[nodesep=3pt]{<-}{R5}{R4}
  \ncline[nodesep=3pt]{<-}{R4}{R3}
  \ncline[nodesep=3pt]{<-}{R4}{R2}
  \ncline[nodesep=3pt]{<-}{R2}{R1} 

\end{figure}


